Inverse-like Antagonistic Scene Text Spotting via Reading-Order Estimation and Dynamic Sampling

Scene text spotting is a challenging task, especially for inverse-like scene text, which has complex layouts, e.g., mirrored, symmetrical, or retro-flexed. In this paper, we propose a unified end-to-end trainable inverse-like antagonistic text spotting framework dubbed IATS, which can effectively spot inverse-like scene texts without sacrificing general ones. Specifically, we propose an innovative reading-order estimation module (REM) that extracts reading-order information from the initial text boundary generated by an initial boundary module (IBM). To optimize and train REM, we propose a joint reading-order estimation loss consisting of a classification loss, an orthogonality loss, and a distribution loss. With the help of IBM, we can divide the initial text boundary into two symmetric control points and iteratively refine the new text boundary using a lightweight boundary refinement module (BRM) for adapting to various shapes and scales. To alleviate the incompatibility between text detection and recognition, we propose a dynamic sampling module (DSM) with a thin-plate spline that can dynamically sample appropriate features for recognition in the detected text region. Without extra supervision, the DSM can proactively learn to sample appropriate features for text recognition through the gradient returned by the recognition module. Extensive experiments on both challenging scene text and inverse-like scene text datasets demonstrate that our method achieves superior performance both on irregular and inverse-like text spotting.

==> 0_abstract.tex <==
\begin{abstract}
For example.

\newif\ifib
\ibtrue%\ibfalse%
\ifib
AHHHHHH
\else
BBBBBB
\fi
\end{abstract}

==> fig_tex/backone.tex <==
\begin{figure}[tbp]
	\begin{center}
	\includegraphics[width=0.96\linewidth]{fig/backone}
		\caption{Architecture of our backbone for feature extraction. $ F_{S} $ denotes the shared features and $ F_p $ denotes the prior information (\ie, classification map, distance field, and direction field).}	
	\label{fig:backbone}
	\end{center}%
\vspace{-1.8em}
\end{figure}


==> fig_tex/fig_ComplexLayout.tex <==
\begin{figure*}[ht]
	\begin{center}
	\subfigure[]{
		\begin{minipage}[t]{0.19\linewidth}
			\centering
			\includegraphics[width=3.5cm,height=2.8cm]{fig/img-order/total-img643}
			%\caption{fig1}
		\end{minipage}%
	}%
	\subfigure[]{
		\begin{minipage}[t]{0.19\linewidth}
			\centering
			\includegraphics[width=3.4cm,height=2.8cm]{fig/img-order/total-img560}
			%\caption{fig2}
		\end{minipage}%
	}%
	%这个回车键很重要 \quad也可以
	\subfigure[]{
		\begin{minipage}[t]{0.19\linewidth}
			\centering
			\includegraphics[width=3.6cm,height=2.8cm]{fig/img-order/0000443}
			%\caption{fig2}
		\end{minipage}
	}%
	\subfigure[]{
		\begin{minipage}[t]{0.19\linewidth}
			\centering
			\includegraphics[width=3.6cm,height=2.8cm]{fig/img-order/0000178}
			%\caption{fig2}
		\end{minipage}
	}%
	\subfigure[]{
	\begin{minipage}[t]{0.19\linewidth}
		\centering
		\includegraphics[width=3.6cm,height=2.8cm]{fig/img-order/0000281}
		%\caption{fig2}
	\end{minipage}
   }%
	\caption{Examples of labels with text reading direction. (a)-(b) are gained from Total-Text, and (c)-(d) are gained from {Inverse-Text}~\cite{DPText}. For each text boundary, the first point is marked as yellow circle, and the remaining points follow the direction indicated by the purple point.}
	\label{fig:layout}
	\end{center}
\vspace{-2.0em}
\end{figure*}

==> tab_tex/tbArT.tex <==
\begin{table}[tbp]
	\begin{center}%\centering
	\renewcommand{\arraystretch}{1.3}
	\caption{Comparisons with related works on ICDAR-ArT. Some experimental result are from \cite{PCR}}
	\label{table:ArT}
	\begin{tabular}{c|c|c|ccc}
		\hline
		\textbf{Methods}&\textbf{Published}&Ext& \textbf{R}& \textbf{P} & \textbf{F}\\
		\hline
		TextRay(Res50) \cite{TextRay}&MM'20&$ \checkmark $ &58.60 &75.97 &66.17\\ 
		%\hline
		PCR(DLA-34) \cite{PCR} &CVPR'21&$ \times $&65.0 &83.6 &73.1\\
		PCR(DLA-34) \cite{PCR} &CVPR'21&$ \checkmark $&66.1 &84.0 &74.0\\
		EMA(DLA-34)\cite{EMA}&TIP'22&$ \checkmark $&68.7&80.8&74.3\\
		%\hline
		\hline
		\hline
		%\textbf{Ours}(Res18-4s) &-&$ \checkmark $&-&- &-\\
		\textbf{Ours}(Res50-1s) &-&$ \checkmark $&71.07&81.14 &75.77\\
		\textbf{Ours}(Res50-1s$ ^{*} $) &-&$ \checkmark $&\textbf{77.05}&\textbf{84.48}&\textbf{80.59}\\
		\hline
	\end{tabular}
    \end{center}%
\vspace{-1.5em}
\end{table}
%\vtop{\hbox{\strut A}\hbox{\strut B}}
%The symbol $ ^{\dagger}$ indicates that the backbone network is not VGG16.
